AFL-Net: Integrating Audio, Facial, and Lip Modalities with a Two-step Cross-attention for Robust Speaker Diarization in the Wild

Speaker diarization in real-world videos presents significant challenges due to varying acoustic conditions, diverse scenes, the presence of off-screen speakers, etc. This paper builds upon a previous study (AVR-Net) and introduces a novel multi-modal speaker diarization system, AFL-Net. The proposed AFL-Net incorporates dynamic lip movement as an additional modality to enhance the identity distinction. Besides, unlike AVR-Net which extracts high-level representations from each modality independently, AFL-Net employs a two-step cross-attention mechanism to sufficiently fuse different modalities, resulting in more comprehensive information to enhance the performance. Moreover, we also incorporated a masking strategy during training, where the face and lip modalities are randomly obscured. This strategy enhances the impact of the audio modality on the system outputs. Experimental results demonstrate that AFL-Net outperforms state-of-the-art baselines, such as the AVR-Net and DyViSE.

==> speaker-diarization/5-limitations.tex <==
\section{Limitations}
\label{sec:limitations}
The proposed method AFL-Net has achieved promising results.
However, speaker diarization under wild conditions still poses significant challenges, including: 
(1) High DER in the wild: Efforts to address visual feature absence are ongoing, especially in complex scenarios. Errors in speaker identification persist even in ideal conditions.
(2) Deployment challenges: AFL-Net focuses on diarization, requiring separate tasks like active speaker and speech detection. Accuracy in these pre-processing tasks crucially impacts final results.
Therefore, achieving a robust end-to-end audio-visual speaker diarization system is our future objective.
